Ranking with submodular functions on a budget

Submodular maximization has been the backbone of many important machine-learning problems, and has applications to viral marketing, diversification, sensor placement, and more. However, the study of maximizing submodular functions has mainly been restricted in the context of selecting a set of items. On the other hand, many real-world applications require a solution that is a ranking over a set of items. The problem of ranking in the context of submodular function maximization has been considered before, but to a much lesser extent than item-selection formulations. In this paper, we explore a novel formulation for ranking items with submodular valuations and budget constraints. We refer to this problem as max-submodular ranking (MSR). In more detail, given a set of items and a set of non-decreasing submodular functions, where each function is associated with a budget, we aim to find a ranking of the set of items that maximizes the sum of values achieved by all functions under the budget constraints. For the MSR problem with cardinality- and knapsack-type budget constraints we propose practical algorithms with approximation guarantees. In addition, we perform an empirical evaluation, which demonstrates the superior performance of the proposed algorithms against strong baselines.

==> legacy.tex <==

\section{Notes about weighted greedy}

\note{Some remarks about the proof.
\begin{itemize}
	\item Some ideas about how to come up the distribution scheme: 
	Regarding the values of $\dup_{jk}$, we consider the demand from each function $\fsm_i$.
	We need $\vopt_1,\ldots,\vopt_{\bg_i}$ to make up for $\fsm_i(\rkopt_{\bg_i})$ in \OPT.
	For a fixed $\vopt_k$, function $\fsm_i$ collects $\dup_{jk}$ portion of $\vopt_k$ at iteration $j \in [\bg_i]$ in which it appears.
	Function $\fsm_i$ with $\bg_i=1$ only appears in iteration $j=1$, so it does not make sense to distribute $\dup_1$ among $\dup_{1k}$ with large $k$.
	Thus we try $\dup_{11}=\dup_1=1$.
	Generally, function $\fsm_i$ can only collect $\vopt_{\bg_i}$ at iteration $j=\bg_i$, while it is able to collect $\vopt_k$ with a smaller $k$ from previous iterations.
	Thus it makes sense to allocate most of $\dup_j$ to $\dup_{jj}$.
	Intuitively, 
	\item The distribution $\dup_{jk}$ is not optimal, but should be asymtopically optimal as $\bgmax = \max_i \bg_i$ increases. 
	There seems little room to be improved in this respect. 
	I didn't find a way to compute the minimum coefficient, as an LP is involved.
	When $\bgmax=2$, the optimal lower bound is around $3/4$, and when $\bgmax=3$, the optimal lower bound is around $5/8$.
	\item Attempts for $\coef_{ij} = \frac{1}{\bg_i-j+1}$ do not seem to give advantage.
	In this case, $\dup_j = 1$ to make LHS easy to upper bound.
	Then we need to decide a distribution scheme $\dup_{jk}$ such that $\sum_{k \in [\nV]}\dup_{jk} = 1, \forall j$.
	A natural choice is geometric series, i.e., $\dup_{jj}=\frac12, \dup_{j,j-1}=\frac14, \ldots, \dup_{j2}=\dup_{j,1}=\frac1{2^{j-1}}$.
	For a fixed $\bg_i=\bg$, study the minimum coefficient
	$\min_{k \in [\bg_i]} \sum_{j \in [\bg_i]} \dup_{jk} \coef_{ij}$.
	Fix $k=1$, $\sum_{j \in [\bg_i]} \dup_{jk} \coef_{ij}$ where $\coef_{ij}$ increases as $j$ increases, i.e., 
	$\frac{1}{\bg}, \frac{1}{\bg-1}, \ldots, \frac{1}{1}$, 
	so we have 
	$\sum_{j \in [\bg_i]} \dup_{jk} \coef_{ij} = \frac{1}{\bg} + \frac{1}{\bg-1}\frac12 + \ldots + \frac{1}{1}\frac1{2^{\bg-1}}$,
	which can be arbitrarily small as $\bg$ increases.
\end{itemize}
}


\section{Notes about FPTAS by Nikolaj}

For simplicity, let us define $g(j, c) = \sum_{i | c(v_j) + c \le b_i, 2c(v_j) > b_i} f_i(v_j)$

$g(j, c)$ is the increase of value when adding $v_j$ when the cost of previous items is c.

The DP should be something like

$T(b, j)$ = the smallest cost of items \rk in $v_1, .., v_j$ while $z(\rk) \ge b$

The recursion should be something like

$T(b, j) = \min \left\{ T(b, j - 1), \min_{x | x + g(j, T(x, j - 1)) \ge b} (T(x, j - 1) + c(v_j)) \right\}$

Here is a sketch of the proof that DP works:

Proposition: $T(b,j) =$ the smallest cost of items \rk in $v_1, .., v_j$ while $z(\rk) \ge b$

Proof:

By induction. Let \rk be the optimal permutation for $T(b, j)$.

If $v_j$ not in \rk, then $c(\rk) \le T(b, j - 1)$.

If $v_j$ is in \rk, then let $\rk’$ be the permutation without $v_j$.
Let $x = z(\rk’)$. Then $T(x, j - 1) \le c(\rk’)$
and
$b \le z(\rk) = x + g(j, c(\rk’)) \le x + g(j, T(x, j - 1))$.
Thus
$T(b, j) \le T(x, j - 1) + c(v_j) \le c(\rk’) + c(v_j) = c(\rk)$.

Do note that in DP the order of $v_j$ is fixed. So DP finds the optimal solution for a fixed order of $v_j$s.
but we know that the optimal solution will be ordered by $c(v_j)$.



\newpage
\section{Fair greedy for knapsack constraint}

\begin{theorem}
\label{thm:weighted-knapsack}
Algorithm \ref{alg-dp} with coefficient $\coef_{ij}=\coef_{i}=1/\bg_i$ is ?-approximation for the \msr problem with non-uniform cost.
\begin{proof}
By greedy, we know the following holds for arbitrary item $v \in \V$ in the $j$-th iteration.
\begin{align}
    \sum_{\fsm_i \in \rsd_{j}: \cost(\rk_{j-1})+\cost(u_j) \le \bg_i} \frac{\coef_i}{\cost(u_j)} \fsm_i(u_j \mid \rk_{j-1}) 
    \ge 
    \sum_{\fsm_i \in \rsd_{j}: \cost(\rk_{j-1})+\cost(v) \le \bg_i} \frac{\coef_i}{\cost(v)} \fsm_i(v \mid \rk_{j-1}).
\end{align}

We denote by $v_j$ the $j$-th item of the optimal permutation \rkopt.
The idea is to replace the arbitrary item $v$ with some proper $v_k \in \rkopt$.
In order to make sure every $v_k$ appear in the RHS to make up the total \OPT,
we make $\dup_{j}$ duplicates of the LHS of the above inequality, and distribute the total amount $\dup_{j}$ to the RHS among different $v_k$, with $\dup_{jk}$ for each $k$ such that
$\dup_{j} = \sum_{k \in [\nV]}\dup_{jk}$.

\begin{itemize}
	\item $\dup_j= \cost(\rk_j) \cdot \min \{ \cost(u_j), \cost(\rkopt)/2-\cost(\rk_{j-1}) \}$ if $\cost(\rk_{j-1}) < \cost(\rkopt)/2$, or $\dup_j=0$.
	\item $\dup_{jk} = (\dup_j - \text{length of rkopt before jk overlap /2}) \cdot \min \{ \cost(u_j), \cost(v_k)/2, \cost(\rkopt_{k})/2-\cost(\rk_{j-1}), \cost(\rk_{j})-\cost(\rkopt_{k-1})/2 \}$ 
		if $\cost(\rkopt_{k-1})/2 \le \cost(\rk_{j})$ and $\cost(\rk_{j-1}) \le \cost(\rkopt_{k})/2 \le \cost(\rkopt)/2$,
		or $\dup_{jk}=0$.
\end{itemize}

\begin{align}
	& \sum_{j \in [\nV]} \sum_{\fsm_i \in \rsd_{j}: \cost(\rk_{j-1})+\cost(u_j) \le \bg_i} \frac{\dup_j\coef_i}{\cost(u_j)} \fsm_i(u_j \mid \rk_{j-1}) 
    \\
    &\ge 
    \sum_{j \in [\nV]} \sum_{k \in [\nV]} \sum_{\fsm_i \in \rsd_{j}: \cost(\rk_{j-1})+\cost(v_k) \le \bg_i} \frac{\dup_{jk}\coef_i}{\cost(v_k)} \fsm_i(v_k \mid \rk_{j-1}) 
\end{align}

\note{Some difficulties:
\begin{itemize}
	\item early item $u_j$ is more cost-efficient, but has a lower $\dup_j$.
	\item $\dup_j = \cost(\rk_j) \le \bg_i$ fails to upper bound $\fsm_i$ in \OPT with coef $1/\bg_i$.
	Can we say anything between $\cost(\rk_{\idx_i})$ and $\bg_i$? We seem to need to use $\coef_i = 1/\cost(\rkopt(\idx_i^*))$ instead of $1/\bg_i$.
\end{itemize}
}
\end{proof}
\end{theorem}



\newpage
\section{Some bad examples for knapsack constraint}

\begin{example}[Singleton is insufficient]
We construct an instance where the algorithm returns $\ALG = \frac1\nfsms \OPT$.
The main idea is to starve as many functions as possible.
\begin{itemize}
	\item Consider function $\fsm_i$ with budget $\bg_i=i, \forall i \in [\nfsms]$.
	\item For each function $\fsm_i$, there is a distinct item $v_i$ such that $\fsm_i(v_i)=1$ and $\cost(v_i)=1$ and $\fsm_j(v_i)=0, \forall j \ne i$.
	\item In addition, there is one small item $v_0$ that is the most cost-efficient, i.e., $\cost(v_0)=\epsilon$, and $\sum_i \fsm_i(v_0) = 2\epsilon$.
	\item \ALG returns two solutions: $(v_0, v_1, \ldots, v_\nfsms, \ldots)$ and a singleton $v_1$, and $\ALG=\fsm_1(v_1)=1$.
	\item \OPT is $(v_1, \ldots, v_\nfsms, \ldots)$, and $\OPT=\sum_i \fsm_i(v_i)=\nfsms$.
\end{itemize}
\end{example}

\begin{example}[Greedy 2nd solution is insufficient]
We construct an instance where the algorithm returns $\ALG = \frac2\nfsms \OPT$.
The main idea is to introduce exclusive greedy large items.
\begin{itemize}
	\item Consider function $\fsm_i$ with budget $\bg_i=2^i, \forall i \in [\nfsms]$.
	\item For each function $\fsm_i$, there is a distinct item $v_{i1}$ such that $\fsm_i(v_{i1})=1-\nfsms\epsilon+i\epsilon$ and $\cost(v_{i1})=2^{i}$ and $\fsm_j(v_{i1})=0, \forall j \ne i$.
	Note that every item $v_{i1}$ becomes infeasible for $\fsm_i$ if it is not the first item.
	\item For each function $\fsm_i$, there is a distinct item $v_{i2}$ such that $\fsm_i(v_{i2})=\frac12 \fsm_i(v_{i1}) - \epsilon$ and $\cost(v_{i1})=2^{i-1}$ and $\fsm_j(v_{i2})=0, \forall j \ne i$.
	Note that item $v_{i2}$ is less cost-efficient than item $v_{i1}$, but takes up less budget.
	\item \ALG returns two solutions: $(v_{11}, \ldots, v_{\nfsms1}, \ldots)$ and $(v_{\nfsms1}, \ldots)$, and $\ALG=\fsm_\nfsms(v_{\nfsms1})=1$.
	\item \OPT is $(v_{12}, \ldots, v_{\nfsms2}, \ldots)$, and $\OPT=\sum_i \fsm_i(v_{i2})\approx \frac\nfsms2$.
\end{itemize}
\end{example}



\newpage
\section{Early derivations for greedy with cardinality constraint}

\begin{theorem}
Algorithm \ref{alg} is 2-approximation for the \msr problem.
\begin{proof}
We denote $\rsd_j$ as the set of unsaturated functions at the beginning of the $j$-th iteration, i.e., 
$\rsd_j=\{ \fsm_i \in \fsms: \cost(\rk_{j-1}) < \bg_i \}$.

By greedy, we know the following holds for arbitrary item $v \in \V$ in the $(j+1)$-th iteration.
\begin{align}
    \sum_{\fsm_i \in \rsd_{j+1}} (\fsm_i(\rk_{j+1}) - \fsm_i(\rk_{j})) / \bg_i \ge 
    \sum_{\fsm_i \in \rsd_{j+1}} \fsm_i(v \mid \rk_j) / \bg_i.
\end{align}
The main idea is to manipulate the above inequality, and finally sum up all iterations to complete the proof.
We denote the optimal permutation as $\rkopt$.% and $v_j$ is its $j$-th item.

\begin{align}
    \sum_{\fsm_i \in \rsd_{j+1}} \frac{1}{\bg_i} (\fsm_i(\rk_{j+1}) - \fsm_i(\rk_{j})) &\ge 
    \sum_{\fsm_i \in \rsd_{j+1}} \frac{1}{\bg_i} \fsm_i(v \mid \rk_j) \\
    (j+1) \sum_{\fsm_i \in \rsd_{j+1}} \frac{1}{\bg_i} (\fsm_i(\rk_{j+1}) - \fsm_i(\rk_{j})) &\ge 
    \sum_{v \in \rkopt_{j+1}} \sum_{\fsm_i \in \rsd_{j+1}} \frac{1}{\bg_i} \fsm_i(v \mid \rk_j) \\
    &= 
    \sum_{\fsm_i \in \rsd_{j+1}} \frac{1}{\bg_i} \sum_{v \in \rkopt_{j+1}} \fsm_i(v \mid \rk_j) \\
    &\ge 
    \sum_{\fsm_i \in \rsd_{j+1}} \frac{1}{\bg_i} (\fsm_i(\rkopt_{j+1} \cup \rk_j) - \fsm_i(\rk_j)) \\
    &\ge 
    \sum_{\fsm_i \in \rsd_{j+1}} \frac{1}{\bg_i} (\fsm_i(\rkopt_{j+1}) - \fsm_i(\rk_j)) \\
    \sum_{\fsm_i \in \rsd_{j+1}} \frac{j+1}{\bg_i} \fsm_i(\rk_{j+1}) - \frac{j}{\bg_i} \fsm_i(\rk_{j}) &\ge 
    \sum_{\fsm_i \in \rsd_{j+1}} \frac{1}{\bg_i} \fsm_i(\rkopt_{j+1})
\end{align}

Now we sum up the above inequality for all iterations.
Note that $\rsd_1 = \fsms$.

\begin{align}
    \sum_{j=0}^{\nV-1} \sum_{\fsm_i \in \rsd_{j+1}} \frac{j+1}{\bg_i} \fsm_i(\rk_{j+1}) - \frac{j}{\bg_i} \fsm_i(\rk_{j}) &\ge 
    \sum_{j=0}^{\nV-1} \sum_{\fsm_i \in \rsd_{j+1}} \frac{1}{\bg_i} \fsm_i(\rkopt_{j+1}).
\end{align}
\begin{align}
    \text{LHS} &= 
    \sum_{j=0}^{\nV-1} \sum_{\fsm_i \in \rsd_{j+1}} \frac{j+1}{\bg_i} \fsm_i(\rk_{j+1}) - \frac{j}{\bg_i} \fsm_i(\rk_{j}) \\
    &= \sum_{\fsm_i \in \fsms} \sum_{j=0}^{\bg_i-1} \left( \frac{j+1}{\bg_i} \fsm_i(\rk_{j+1}) - \frac{j}{\bg_i} \fsm_i(\rk_{j}) \right) \\
    &= \sum_{\fsm_i \in \fsms} \fsm_i(\rk_{\bg_i}) 
    = \ALG.
\end{align}

In the worst case, 
$\fsm_i(\rkopt_j) = 0$ for all $j < \bg_i$, so
$\sum_{j=1}^{\bg_i} \fsm_i(\rkopt_j) = \fsm_i(\rkopt_{\bg_i})$.
\begin{align}
    \text{RHS} &= 
    \sum_{\fsm_i \in \fsms} \frac{1}{\bg_i} \sum_{j=1}^{\bg_i} \fsm_i(\rkopt_j) 
    \ge \sum_{\fsm_i \in \fsms} \frac{1}{\bg_i} \fsm_i(\rkopt_{\bg_i})
    \\
    & \ge \min_i \frac{1}{\bg_i} \sum_{\fsm_i \in \fsms} \fsm_i(\rkopt_{\bg_i}) = \OPT / \nV
\end{align}


\note{LHS needs a (nearly) telescoping series keep only $\fsm_i(\rk_{\bg_i})$ for each $i$.
RHS needs to provide toughly a fraction $\frac 1{\bg_i} \fsm_i(\rkopt_{\bg_i})$ for each $i \in \rsd_j $ in each iteration to make up a whole $\fsm_i(\rkopt_{\bg_i})$.}

Old: Both sides times $n$ instead of $j+1$.


\begin{align}
    \sum_{\fsm_i \in \rsd_{j+1}} \frac{1}{\bg_i} (\fsm_i(\rk_{j+1}) - \fsm_i(\rk_{j})) &\ge 
    \sum_{\fsm_i \in \rsd_{j+1}} \frac{1}{\bg_i} \fsm_i(v \mid \rk_j) \\
    \nV \sum_{\fsm_i \in \rsd_{j+1}} \frac{1}{\bg_i} (\fsm_i(\rk_{j+1}) - \fsm_i(\rk_{j})) &\ge 
    \sum_{v \in \rkopt} \sum_{\fsm_i \in \rsd_{j+1}} \frac{1}{\bg_i} \fsm_i(v \mid \rk_j) \\
    &= 
    \sum_{\fsm_i \in \rsd_{j+1}} \frac{1}{\bg_i} \sum_{v \in \rkopt} \fsm_i(v \mid \rk_j) \\
    &\ge 
    \sum_{\fsm_i \in \rsd_{j+1}} \frac{1}{\bg_i} (\fsm_i(\rkopt \cup \rk_j) - \fsm_i(\rk_j)) \\
    &\ge 
    \sum_{\fsm_i \in \rsd_{j+1}} \frac{1}{\bg_i} (\fsm_i(\rkopt) - \fsm_i(\rk_j)) \\
    \sum_{\fsm_i \in \rsd_{j+1}} \frac{\nV}{\bg_i} \fsm_i(\rk_{j+1}) - (\frac{\nV}{\bg_i} - \frac{1}{\bg_i}) \fsm_i(\rk_{j})) &\ge 
    \sum_{\fsm_i \in \rsd_{j+1}} \frac{1}{\bg_i} \fsm_i(\rkopt)
\end{align}

\begin{align}
    \sum_{j=0}^{\nV-1} \sum_{\fsm_i \in \rsd_{j+1}} \frac{\nV}{\bg_i} \fsm_i(\rk_{j+1}) - (\frac{\nV}{\bg_i} - \frac{1}{\bg_i}) \fsm_i(\rk_{j})) &\ge 
    \sum_{j=0}^{\nV-1} \sum_{\fsm_i \in \rsd_{j+1}} \frac{1}{\bg_i} \fsm_i(\rkopt) \\
    &= 
    \sum_{\fsm_i \in \fsms} \bg_i \frac{1}{\bg_i} \fsm_i(\rkopt) \\
    &= 
    \sum_{\fsm_i \in \fsms} \fsm_i(\rkopt) \\
    &\ge 
    \OPT \\
    \sum_{j=0}^{\nV-1} \sum_{\fsm_i \in \rsd_{j+1}} \frac{\nV}{\bg_i} \fsm_i(\rk_{j+1}) - (\frac{\nV}{\bg_i} - \frac{1}{\bg_i}) \fsm_i(\rk_{j})) &\ge 
    \OPT \\
    \sum_{\fsm_i \in \fsms} \sum_{j=0}^{\bg_i-1} \left( \frac{\nV}{\bg_i} \fsm_i(\rk_{j+1}) - (\frac{\nV}{\bg_i} - \frac{1}{\bg_i}) \fsm_i(\rk_{j})) \right) &\ge 
    \OPT \\
    \sum_{\fsm_i \in \fsms} \sum_{j=0}^{\bg_i-1} \left( \frac{\nV}{\bg_i} \fsm_i(\rk_{j+1}) - (\frac{\nV}{\bg_i} - \frac{1}{\bg_i}) \fsm_i(\rk_{j})) \right) &\ge 
    \OPT \\
\end{align}

If not divided 1/bi

\begin{align}
    \sum_{\fsm_i \in \rsd_{j+1}}  (\fsm_i(\rk_{j+1}) - \fsm_i(\rk_{j})) &\ge 
    \sum_{\fsm_i \in \rsd_{j+1}} \fsm_i(v \mid \rk_j) \\
    (j+1) \sum_{\fsm_i \in \rsd_{j+1}}  (\fsm_i(\rk_{j+1}) - \fsm_i(\rk_{j})) &\ge 
    \sum_{v \in \rkopt_{j+1}} \sum_{\fsm_i \in \rsd_{j+1}} \fsm_i(v \mid \rk_j) \\
    &= 
    \sum_{\fsm_i \in \rsd_{j+1}} \frac{1}{\bg_i} \sum_{v \in \rkopt_{j+1}} \fsm_i(v \mid \rk_j) \\
    &\ge 
    \sum_{\fsm_i \in \rsd_{j+1}} (\fsm_i(\rkopt_{j+1} \cup \rk_j) - \fsm_i(\rk_j)) \\
    &\ge 
    \sum_{\fsm_i \in \rsd_{j+1}} (\fsm_i(\rkopt_{j+1}) - \fsm_i(\rk_j)) \\
    \sum_{\fsm_i \in \rsd_{j+1}} (j+1) \fsm_i(\rk_{j+1}) - j \fsm_i(\rk_{j}) &\ge 
    \sum_{\fsm_i \in \rsd_{j+1}} \fsm_i(\rkopt_{j+1})
\end{align}


\end{proof}
\end{theorem}

